Fluent Logic Workflow Analyser: A Tool for The Verification of Workflow Properties

In this paper we present the design and implementation, as well as a use case, of a tool for workflow analysis. The tool provides an assistant for the specification of properties of a workflow model. The specification language for property description is Fluent Linear Time Temporal Logic. Fluents provide an adequate flexibility for capturing properties of workflows. Both the model and the properties are encoded, in an automated way, as Labelled Transition Systems, and the analysis is reduced to model checking.

==> eptcsdata.tex <==
\providecommand{\firstpage}{46}
\providecommand{\publicationstatus}{Nazareno Aguirre, Leila Ribeiro (Eds.):\\
First Latin American Workshop on Formal Methods (LAFM 2013)\\
EPTCS 139, 2014, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.139.4}{10.4204/EPTCS.139.4}}
\pdfoutput=1

